Testable Learning with Distribution Shift

We revisit the fundamental problem of learning with distribution shift, in which a learner is given labeled samples from training distribution $D$, unlabeled samples from test distribution $D'$ and is asked to output a classifier with low test error. The standard approach in this setting is to bound the loss of a classifier in terms of some notion of distance between $D$ and $D'$. These distances, however, seem difficult to compute and do not lead to efficient algorithms. We depart from this paradigm and define a new model called testable learning with distribution shift, where we can obtain provably efficient algorithms for certifying the performance of a classifier on a test distribution. In this model, a learner outputs a classifier with low test error whenever samples from $D$ and $D'$ pass an associated test; moreover, the test must accept if the marginal of $D$ equals the marginal of $D'$. We give several positive results for learning well-studied concept classes such as halfspaces, intersections of halfspaces, and decision trees when the marginal of $D$ is Gaussian or uniform on $\{\pm 1\}^d$. Prior to our work, no efficient algorithms for these basic cases were known without strong assumptions on $D'$. For halfspaces in the realizable case (where there exists a halfspace consistent with both $D$ and $D'$), we combine a moment-matching approach with ideas from active learning to simulate an efficient oracle for estimating disagreement regions. To extend to the non-realizable setting, we apply recent work from testable (agnostic) learning. More generally, we prove that any function class with low-degree $L_2$-sandwiching polynomial approximators can be learned in our model. We apply constructions from the pseudorandomness literature to obtain the required approximators.

==> ns2_preliminaries.tex <==
\section{Preliminaries}

\subsection{Notation and Basic Definitions}
% We let $\X\subseteq \R^d$ and, in particular, $\X$ will either be the $d$-dimensional hypercube $\cube{d}$ or the $d$-dimensional Euclidean space $\R^d$. For a distribution $\Dgeneric$ over $\X$, we use $\E_\Dgeneric$ (or $\E_{\x\sim \Dgeneric}$) to refer to the expectation over distribution $\Dgeneric$ and for a given (multi)set $\Sunlabelled$, we use $\E_\Sunlabelled$ (or $\E_{\x\sim \Sunlabelled}$) to refer to the expectation over the uniform distribution on $\Sunlabelled$ (i.e., $\E_{\x\sim \Sunlabelled}[g(\x)] = \frac{1}{|\Sunlabelled|}\sum_{\x\in \Sunlabelled}g(\x)$, counting possible duplicates separately). We let $\R_+ = (0,\infty)$. 

% For a function $p:\X\to \R$ and $r\in\N$, we define the $\L_r$ norm of $p$ under $\Dgeneric$ as $\|p\|_{\L_r(\Dgeneric)} = {\ex_{\x\sim \Dgeneric}[p(\x)^r]}^{{1}/{r}}$. %Similarly, we define the $L_1$ norm of $p$ under $\Dgeneric$ as $\|p\|_{L_1(\Dgeneric)} = {\ex_{\x\sim \Dgeneric}[|p(\x)|]}$. %When the distribution $\Dgeneric$ is clear by the context, we may instead use the notation $\|p\|_2$ and $\|p\|_1$ in place of $\|p\|_{\L_2(\Dgeneric)}$ and $\|p\|_{L_1(\Dgeneric)}$ correspondingly. 
% For $\x\in \X$ where $\x = (\x_1,\x_2,\dots,\x_d)$ and for $\mindex \in \N^d$, we denote with $\x^\mindex$ the product $\prod_{i\in[d]}\x_i^{\mindex_i}$, $\moment_\mindex = \E[\x^\mindex]$ and $\|\mindex\|_1 = \sum_{i\in[d]}\mindex_i$. For a polynomial $p$ over $\R^d$ and $\mindex\in \N^d$, we denote with $p_\mindex$ the coefficient of $p$ corresponding to $\x^\mindex$, i.e., we have $p(\x) = \sum_{\mindex\in\N^d}p_\mindex \x^\mindex$. If $p$ is a polynomial over $\cube{d}$, then we can always express it in a unique multilinear form, so we will only use coefficients $p_\mindex$ with $\mindex \in \{0,1\}^d$, i.e., $p(\x) = \sum_{\mindex\in \{0,1\}^d} p_\mindex \x^\mindex$. We define the degree of $p$ and denote $\deg(p)$ the maximum degree of a monomial whose coefficient in $p$ is non-zero, i.e., $\deg(p) = \max\{\|\mindex\|_1: p_\mindex \neq 0\}$. 

% We denote with $\S^{d-1}$ the $d-1$ dimensional sphere on $\R^d$. For any $\vv_1,\vv_2\in\R^d$, we denote with $\vv_1\cdot \vv_2 $ the inner product between $\vv_1$ and $\vv_2$ and we let $\measuredangle (\vv_1,\vv_2)$ be the angle between the two vectors, i.e., the quantity $\theta\in [0,\pi]$ such that $\|\vv_1\|_2\|\vv_2\|_2\cos(\theta) = \vv_1\cdot \vv_2$. For $\vv\in\R^d,\tau\in \R$, we call a function of the form $\x\mapsto \sign(\vv\cdot \x)$ an origin-centered (or homogeneous) halfspace and a function of the form $\x\mapsto \sign(\vv\cdot \x - \tau)$ a general halfspace over $\R^d$. 

% \paragraph{$\L_2$ sandwiching degree.} We now define the notion of $\L_2$ sandwiching polynomials for a function $\concept$ with respect to a distribution $\Dgeneric$, i.e., a pair of polynomials such that one of them is pointwise above $\concept$, the other one is pointwise below $\concept$ and the $\L_2$ distance between the two polynomials with respect to $\Dgeneric$ is small. While the notion of $L_1$ sandwiching polynomials is standard in the literature of pseudorandomness (see, e.g., \cite{bazzi2009polylogarithmic}) and has applications to testable learning (see \cite{gollakota2023efficient}), in order to acquire our main results, we make use of the stronger notion of $\L_2$ sandwiching polynomials which we define below.

% \begin{definition}[$\L_2$ sandwiching polynomials]\label{definition:l2-sandwiching}
%     Consider a product set $\X$ and a distribution $\Dgeneric$ over $\X$. For $\eps>0$ and $\concept:\X\to \cube{}$, we say that the polynomials $\pup, \pdown:\X \to \R$ are $\eps$-approximate $\L_2$ sandwiching polynomials for $\concept$ under $\Dgeneric$ if the following are true.
%     \begin{enumerate}
%         \item $\pdown(\x) \le \concept(\x) \le \pup(\x)$, for all $\x \in \X$.
%         \item $\|\pup-\pdown\|_{\L_2(\Dgeneric)}^2 \le \eps$
%     \end{enumerate}
%     Moreover, for $\eps>0$, a concept class $\C\subseteq\{\X\to \cube{}\}$ and $k,\pbound>0$, we say that the $\eps$-approximate $\L_2$ sandwiching degree of $\C$ under $\Dgeneric$ is at most $k$ and with coefficient bound $\pbound$ if for any $\concept\in\C$ there are $\eps$-approximate $\L_2$ sandwiching polynomials $\pup, \pdown$ for $\concept$ such that $\deg(\pup),\deg(\pdown) \le k$ and each of the coefficients of $\pup,\pdown$ are absolutely bounded by $\pbound$.
% \end{definition}


% \subsection{Learning Setup}

% %\paragraph{Agnostic Setting.} 
% Consider $\Dtrainjoint, \Dtestjoint$ to be distributions over $\X\times \cube{}$ and let $\Dtrainmarginal, \Dtestmarginal$ be the corresponding marginal distributions on $\X$. Our tester-learners receive labelled examples from $\Dtrainjoint$ and unlabelled examples from $\Dtestmarginal$ and their goal is to produce a hypothesis with low error on $\Dtestjoint$ or potentially reject but only if distribution shift is detected. Given a hypothesis class $\C\subseteq\{\X\to \cube{}\}$, $h_1, h_2:\X\to\cube{}$ and distributions $\Dgenericjoint, \Dtrainjoint, \Dtestjoint$ over $\X\times\cube{}$, we define $\error(h_1; \Dgenericjoint) = \pr_{(\x,y)\sim \Dgenericjoint}[y \neq h_1(\x)]$ and $\error(h_1, h_2; \Dgenericmarginal) = \pr_{\x\sim \Dgenericmarginal}[h_1(\x) \neq h_2(\x)]$ as well as the following quantity, which is standard in the domain adaptation literature (see, e.g., \cite{ben2006analysis,blitzer2007learning,ben2010theory,david2010impossibility}).
% \begin{equation}
%     \optcommon(\C;\Dtrainjoint,\Dtestjoint) := \min_{\concept\in \C}\{ \error(\concept; \Dtrainjoint) + \error(\concept; \Dtestjoint)\}, \text{ attained by }\coptcommon\in \C \label{equation:definition:optcommon}
% \end{equation}
% Observe that parameter $\optcommon$ becomes small whenever the training and test errors can be simultaneously minimized by a common classifier in $\C$. Clearly, if there is no relationship between the training and test distributions, then using data from the training distribution does not reveal any information about the test distribution and, therefore, learning is hopeless (see also \Cref{theorem:error-lower-bound-easy}). We will assume (as is common in the domain adaptation literature) that the parameter $\optcommon$ is a valid choice for quantifying the relationship between the training and test distributions, in the sense that considering $\optcommon$ to be small is not unrealistic. In particular, we will partly focus on the following setting where $\optcommon$ is zero. To distinguish between the two settings, we say that we are in the \textbf{agnostic setting} when $\optcommon\ge 0$ (arbitrary) and in the \textbf{realizable setting} when $\optcommon=0$.
% % \begin{align*}
% %     \opttrain &= \min_{\concept\in \C} \error(\concept; \Dtrainjoint), \text{ which is attained by } \copttrain \in \C \\
% %     \opttest &= \min_{\concept\in \C} \error(\concept; \Dtestjoint), \text{ which is attained by } \copttest \in \C 
% % \end{align*}
% % Moreover, we define the following auxiliary quantities.
% % \begin{align*}
% %     \drifttrain = \error(\copttrain, \copttest; \Dtrainmarginal) &\text{ and } \drifttest = \error(\copttrain, \copttest; \Dtestmarginal) \\
% %     \opttesttrain = \error(\copttest; \Dtrainjoint) &\text{ and } \opttraintest = \error(\copttrain; \Dtestjoint)
% % \end{align*}
% % For the following, we denote with $\opt$ the tuple $(\opttrain,\opttest,\drifttrain,\drifttest,\opttesttrain,\opttraintest)$ corresponding to the distributions $\Dtrainjoint$ and $\Dtestjoint$.

% \paragraph{Realizable Setting.} When $\optcommon=0$, there exists a classifier in $\C$ that achieves both zero training loss and test loss and we therefore refer to this setting as realizable. Another (slightly more specific) way to view the realizable setting is by considering the labelled distribution $\Dtrainjoint$ (resp. $\Dtestjoint$) formed as follows: for some $\coptcommon\in \C$, draw an example $\x$ from $\Dtrainmarginal$ (resp. $\Dtestmarginal$) and form the pair $(\x,y) \sim \Dtrainjoint$ (resp. $(\x,y)\sim \Dtestjoint$) by setting $y = \coptcommon(\x)$.
% We now provide a formal definition of our learning model.

% \begin{definition}[Testable Learning under Distribution Shifts (TDS Learning)]
% \label{definition:tds-learning}
%     Let $\X\subseteq \R^d$ and consider a distribution $\Dgeneric$ over $\X$ and a concept class $\C\subseteq\{\X\to \cube{}\}$. For some $\psi:[0,1]\to [0,1]$ and $\eps,\delta\in(0,1)$, we say that an algorithm $\A$ testably learns $\C$ under distribution shifts w.r.t. $\Dgeneric$ up to error $\psi(\optcommon)+\eps$ and probability of failure $\delta$ if the following is true. For any distributions $\Dtrainjoint, \Dtestjoint$ over $\X\times\cube{}$ such that $\Dtrainmarginal = \Dgeneric$, algorithm $\A$, upon receiving a large enough set of labelled samples $\Strain$ from the training distribution $\Dtrainjoint$ and a large enough set of unlabelled samples $\Stest$ from the test distribution $\Dtestmarginal$, either rejects $(\Strain,\Stest)$ or accepts and outputs a hypothesis $h:\X\to \cube{}$ with the following guarantees.
%     \begin{enumerate}[label=\textnormal{(}\alph*\textnormal{)}]
%     \item (Soundness.) With probability at least $1-\delta$ over the samples $\Strain,\Stest$ we have: 
    
%     If $A$ accepts, then the output $h$ satisfies $\error(h;\Dtestjoint) \leq \psi(\optcommon) + \eps$.
%     \item (Completeness.) Whenever $\Dtestmarginal = \Dtrainmarginal$, $A$ accepts with probability at least $1-\delta$ over the samples $\Strain,\Stest$.
%     \end{enumerate}
%     In particular, we say that $\A$ testably learns $\C$ under distribution shifts w.r.t. $\Dgeneric$ in the realizable setting, if $\A$ is required to satisfy the above guarantees only when $\Dtrainjoint,\Dtestjoint$ and $\C$ are realizable (where $\optcommon = 0 = \psi(\optcommon)$).
%     \end{definition}


%\subsection{Auxiliary Tools and Definitions}

% \paragraph{Boosting success probability.} We will now demonstrate that it is possible to boost the probability of success of a TDS learner through repetition. Note that this is not immediate for TDS learning like, for example, in agnostic learning, where one may repeat an agnostic learning algorithm and choose the hypothesis with the smallest error estimate among the outputs of the independent runs. The main obstacle is that test labels are not available. Nonetheless, we obtain the following theorem regarding boosting the probability of success.

% \begin{proposition}[Boosting Success Probability]\label{proposition:boosting-success-probability}
%     Let $\C$ be a hypothesis class, $\Dgeneric$ a distribution and suppose $\A$ is a TDS learner for $\C$ with respect to $\Dgeneric$ with error guarantee $\psi(\optcommon)+\eps$ and failure probability at most $0.1$. Then, there is a TDS learner $\A'$ for $\C$ with respect to $\Dgeneric$ with error guarantee $4\psi(\optcommon)+4\eps$ and failure probability at most $\delta$. In particular, $\A'$ repeats $\A$ for $T = O(\log(\frac{1}{\eps\delta}))$ times and rejects if most of the repetitions reject. If most repetitions accept, $\A'$ outputs the hypothesis $h = \majority(h_1,\dots,h_{T/2})$ ($h$ outputs the majority vote of $h_i$), where $h_1,\dots,h_{T/2}$ are the outputs of the first $T/2$ repetitions of $\A$ that accepted.
% \end{proposition}

% \begin{proof}
%     We split the proof into two parts, one for soundness and one for completeness.
    
%     \paragraph{Soundness.} For soundness, suppose that $\A'$ accepts. We denote with $\hat\pr$ (resp. $\hat\E$) the probabilities (resp. expectations) over the randomness of $h_1,\dots,h_{T/2}$ (which originates to the randomness of the samples given to $\A$) and with $\pr$ (resp. $\E$) the probabilities (resp. expectations) over the randomness of a pair $(\x,y)$ drawn from $\Dtestjoint$. In what follows, let $\eta = \psi(\optcommon)+\eps$. We have that for any $i=1,2,\dots,T/2$, $\hat\pr[\error(h_i,\Dtestjoint)\le \eta] \ge 0.9$, by the guarantees of $\A'$. We will show that $\hat\pr[\error(h,\Dtestjoint)\le 4\eta]\ge 1-\delta$ for a sufficiently large $T=O(\log(\frac{1}{\eps\delta}))$.

%     We define $\goodevent_i$ to be the event (over the randomness of $h_i$) that $h_i$ is `good', i.e., that $\pr[h_i(\x)\neq y] \le \eta$. We define $\badregion$ to be the `bad' region of $(\x,y)$, i.e., $\badregion = \{(\x,y)\in\X\times\cube{}: \hat\pr[h_1(\x)\neq y|\goodevent_1] > 1/3\}$. Note that $\badregion$ would be the same even if we substituted $(h_1,\goodevent_1)$ above with an arbitrary $(h_i,\goodevent_i)$.

%     First, we observe that $\pr[h(\x)\neq y] \le \pr[(\x,y)\in\badregion] + \pr[h(\x)\neq y|(\x,y)\not\in\badregion]$.

%     We now observe that $\pr[(\x,y)\in \badregion] = \pr[\hat\pr[h_1\neq y|\goodevent_1]>1/3] \le 3 \E\hat\pr[h_1(\x)\neq y|\goodevent_1]$ by Markov's inequality. Now, we may swap the expectations to acquire $\pr[(\x,y)\in \badregion] \le 3\hat\E[\pr[h_1(\x)\neq y]|\goodevent_1] \le 3\eta$. 

%     So far, we have shown $\pr[h(\x)\neq y] \le 3\eta + \pr[h(\x)\neq y|(\x,y)\not\in\badregion]$. We will bound the probability over $h_1,\dots,h_{T/2}$ that $\pr[h(\x)\neq y|(\x,y)\not\in\badregion]>\eta$. In particular, we have the following due to Markov's inequality $\hat\pr[\pr[h(\x)\neq y|(\x,y)\not\in\badregion]>\eta] \le \frac{1}{\eta}\hat\E[\pr[h(\x)\neq y|(\x,y)\not\in\badregion]]$. Once more, we may swap the expectations to acquire $\hat\pr[\pr[h(\x)\neq y|(\x,y)\not\in\badregion]>\eta] \le \frac{1}{\eta}\E[\hat\pr[h(\x)\neq y]|(\x,y)\not\in\badregion]$.

%     Moreover, if we fix $(\x,y)\not\in\badregion $, then $\hat\pr[h_i(\x)=y] \ge \hat\pr[h_i(\x)=y \text{ and } \goodevent_i] \ge \frac{2}{3}\cdot \frac{9}{10} \ge 3/5$. Because $\hat\pr[\goodevent_i]\ge 0.9$ and $\hat\pr[h_i(\x)=y | \goodevent_i] \ge 2/3$ whenever $(\x,y)\not\in\badregion$, by the definition of $\badregion$. Therefore, since $h_1,\dots,h_{T/2}$ are independent, we have that $\hat\pr[h(\x)\neq y] \le \exp(-T/C)$ for some sufficiently large universal constant $C>0$, for any $(\x,y)\not\in\badregion$.

%     Therefore, in total, $\hat\pr[\pr[h(\x)\neq y|(\x,y)\not\in\badregion]>\eta] \le \frac{1}{\eta}\exp(-T/C)$. We set $T = C\ln(\frac{1}{\eps\delta}) \ge C\ln(\frac{1}{\eta\delta})$ to obtain $\hat\pr[\pr[h(\x)\neq y|(\x,y)\not\in\badregion]>\eta] \le \delta$ and, hence, with probability at least $1-\delta$ over the randomness of $h$ we overall have $\pr[h(\x)\neq y]\le 4\eta$.
    
%     \paragraph{Completeness.} Completeness follows by a standard Hoeffding bound.
% \end{proof}

% \paragraph{$\L_2$ sandwiching degree.} We now define the notion of $\L_2$ sandwiching polynomials for a function $\concept$ with respect to a distribution $\Dgeneric$, i.e., a pair of polynomials such that one of them is pointwise above $\concept$, the other one is pointwise below $\concept$ and the $\L_2$ distance between the two polynomials with respect to $\Dgeneric$ is small. While the notion of $L_1$ sandwiching polynomials is standard in the literature of pseudorandomness (see, e.g., \cite{bazzi2009polylogarithmic}) and has applications to testable learning (see \cite{gollakota2023efficient}), in order to acquire our main results, we make use of the stronger notion of $\L_2$ sandwiching polynomials which we define below.

% \begin{definition}[$\L_2$ sandwiching polynomials]\label{definition:l2-sandwiching}
%     Consider a product set $\X$ and a distribution $\Dgeneric$ over $\X$. For $\eps>0$ and $\concept:\X\to \cube{}$, we say that the polynomials $\pup, \pdown:\X \to \R$ are $\eps$-approximate $\L_2$ sandwiching polynomials for $\concept$ under $\Dgeneric$ if the following are true.
%     \begin{enumerate}
%         \item $\pdown(\x) \le \concept(\x) \le \pup(\x)$, for all $\x \in \X$.
%         \item $\|\pup-\pdown\|_{\L_2(\Dgeneric)}^2 \le \eps$
%     \end{enumerate}
%     Moreover, for $\eps>0$, a concept class $\C\subseteq\{\X\to \cube{}\}$ and $k,\pbound>0$, we say that the $\eps$-approximate $\L_2$ sandwiching degree of $\C$ under $\Dgeneric$ is at most $k$ and with coefficient bound $\pbound$ if for any $\concept\in\C$ there are $\eps$-approximate $\L_2$ sandwiching polynomials $\pup, \pdown$ for $\concept$ such that $\deg(\pup),\deg(\pdown) \le k$ and each of the coefficients of $\pup,\pdown$ are absolutely bounded by $\pbound$.
% \end{definition}

% \paragraph{Properties of Gaussian and Uniform Distributions.} Let $\Gauss(0,I_d)$ denote the standard multivariate Gaussian distribution over $\R^d$ and $\Unif(\cube{d})$ denote the uniform distribution over the hypercube $\cube{d}$. We will make use of the following simple facts about these distributions, whose proofs (and slightly more quantified versions) can be found in \Cref{appendix:auxiliary-propositions}.

% In particular, we show that the sandwiching polynomials of any binary concept have coefficients that are absolutely bounded, that the empirical moments concentrate around the true ones and that the empirical squared error of polynomials with bounded degree and coefficients uniformly converges to the true squared error.

% \begin{lemma}[Properties of the Gaussian and Uniform Distributions]\label{lemma:gaussian-uniform-properties}
%     Let $\Dgeneric$ be the standard Gaussian $\Gauss(0,I_d)$ over $\R^d$ or the uniform distribution over $\cube{d}$. Then the following are true.
%     \begin{enumerate}[label=\textnormal{(}\roman*\textnormal{)}]
%         \item%\label{item:gaussian-coefficient-bound} 
%         (Coefficient Bound) If $\pup,\pdown$ are $1$-approximate $\L_2(\Dgeneric)$ sandwiching polynomials of degree $\degbound$ for some binary valued function, then their coefficients are absolutely bounded by $\pbound=O(d)^\degbound$.
%         \item%\label{item:gaussian-concentration} 
%         (Moment Concentration)
%         If $\Sunlabelled\sim\Dgeneric^{\otimes m}$ with $m \ge \mconc = \frac{O(d\degbound)^{\degbound}}{\Delta^2\delta}$, then with probability at least $1-\delta$ we have that for any $\mindex\in \N^d$ with $\|\mindex\|_1\le k$ it holds $|\E_\Sunlabelled[\x^\mindex] - \E_\Dgeneric[\x^\mindex]| \le \Delta$.
%         \item%\label{item:gaussian-generalization} 
%         (Generalization) 
%         If $\Slabelled\sim\Dgenericjoint^{\otimes m}$ for some distribution $\Dgenericjoint$ with $\Dgenericmarginal = \Dgeneric$ and $m \ge \mgen = \tilde{O}(\frac{\pbound^8}{\eps^4\delta})\cdot d^{O(\degbound)}$, then with probability at least $1-\delta$ we have that for any degree $k$ polynomial with coefficient bound $B$ it holds $|\E_\Slabelled[(y-p(\x))^2]-\E_{\Dgenericjoint}[(y-p(\x))^2]|\le {\eps}$.
%     \end{enumerate}
% \end{lemma}


==> ns7_discussion.tex <==
\section{Discussion}

-- Connection to Testable learning: do not make assumptions about the training distribution, but test them. Our results extend to this case.\\
-- Universal TDS learning. Some of our results extend to this setting, but it is interesting to see other results.\\
-- Mention perturbations-based learning under covariate shifts and adversarially robust learning. \\
-- Future direction: small number of test labels available.
